Using Battery Storage for Peak Shaving and Frequency Regulation: Joint Optimization for Superlinear Gains

We consider using a battery storage system simultaneously for peak shaving and frequency regulation through a joint optimization framework which captures battery degradation, operational constraints and uncertainties in customer load and regulation signals. Under this framework, using real data we show the electricity bill of users can be reduced by up to 15\%. Furthermore, we demonstrate that the saving from joint optimization is often larger than the sum of the optimal savings when the battery is used for the two individual applications. A simple threshold real-time algorithm is proposed and achieves this super-linear gain. Compared to prior works that focused on using battery storage systems for single applications, our results suggest that batteries can achieve much larger economic benefits than previously thought if they jointly provide multiple services.

==> bio.tex <==
% Yuanyuan Shi
\begin{IEEEbiography}
	[
	{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{yuanyuan.eps}}
	] {Yuanyuan Shi} received her Bachelor of Engineering in Automation from Nanjing Univeristy, China in 2015. She is currently pursuing her Ph.D. degree in Electrical Engineering and M.S. in Statistics at the University of Washington, Seattle, WA, USA.

	She works on optimization, control and machine learning, with applications in power systems and cyberphysical systems. She is a recipient of Washington Clean Energy Institute graduate fellowship on energy and sustainability.
\end{IEEEbiography}

% Bolun Xu
\begin{IEEEbiography}[
	{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bolun.eps}}]{Bolun Xu}
	(S'14) received B.S. degrees in Electrical and Computer Engineering from the University of Michigan, Ann Arbor, USA and Shanghai Jiaotong University, Shanghai, China in 2011, and the M.Sc degree in Electrical Engineering from Swiss Federal Institute of Technology, Zurich, Switzerland in 2014. He is currently pursuing the Ph.D. degree in Electrical Engineering at the University of Washington, Seattle, WA, USA. His research interests include energy storages, power system operations, and power system economics.
\end{IEEEbiography}

%% Di Wang
\begin{IEEEbiography}
	[
	{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{di.eps}}
	] {Di Wang} is a researcher at Microsoft. He received his B.E. in Computer Science and Technology from Zhejiang University (2005), M.S. in Computer Systems Engineering from Technical University of Denmark (2008), and Ph.D. in Computer Science and Engineering from The Pennsylvania State University (2014). His research spans the areas of computer systems, computer architecture, software-hardware interface, and energy efficient system design and management.
\end{IEEEbiography}

% Baosen Zhang
\begin{IEEEbiography}
	[
	{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{baosen.eps}}
	] {Baosen Zhang} received his Bachelor of Applied Science in Engineering Science degree from the University of Toronto in 2008; and his PhD degree in Electrical Engineering and Computer Sciences from University of California, Berkeley in 2013.

	He was a Postdoctoral Scholar at Stanford University, affiliated with the Civil and Environmental Engineering and Management \& Science Engineering. He is currently an Assistant Professor in Electrcial Engineering at the University of Washington, Seattle, WA. His research interests are in power systems and cyberphysical systems. He was selected as one of Forbe's 30 under 30 in energy in 2015.
\end{IEEEbiography}

